Caruca: Effective and Efficient Specification Mining for Opaque Software Components

A wealth of state-of-the-art systems demonstrate impressive improvements in performance, security, and reliability on programs composed of opaque components, such as Unix shell commands. To reason about commands, these systems require partial specifications. However, creating such specifications is a manual, laborious, and error-prone process, limiting the practicality of these systems. This paper presents Caruca, a system for automatic specification mining for opaque commands. To overcome the challenge of language diversity across commands, Caruca first instruments a large language model to translate a command's user-facing documentation into a structured invocation syntax. Using this representation, Caruca explores the space of syntactically valid command invocations and execution environments. Caruca concretely executes each command-environment pair, interposing at the system-call and filesystem level to extract key command properties such as parallelizability and filesystem pre- and post-conditions. These properties can be exported in multiple specification formats and are immediately usable by existing systems. Applying Caruca across 60 GNU Coreutils, POSIX, and third-party commands across several specification-dependent systems shows that Caruca generates correct specifications for all but one case, completely eliminating manual effort from the process and currently powering the full specifications for a state-of-the-art static analysis tool.

==> misc.tex <==
% taken from manual
\makeatletter
\pgfdeclareshape{document}{
\inheritsavedanchors[from=rectangle] % this is nearly a rectangle
\inheritanchorborder[from=rectangle]
\inheritanchor[from=rectangle]{center}
\inheritanchor[from=rectangle]{north}
\inheritanchor[from=rectangle]{south}
\inheritanchor[from=rectangle]{west}
\inheritanchor[from=rectangle]{east}
% ... and possibly more
\backgroundpath{% this is new
% store lower right in xa/ya and upper right in xb/yb
\southwest \pgf@xa=\pgf@x \pgf@ya=\pgf@y
\northeast \pgf@xb=\pgf@x \pgf@yb=\pgf@y
% compute corner of ‘‘flipped page’’
\pgf@xc=\pgf@xb \advance\pgf@xc by-10pt % this should be a parameter
\pgf@yc=\pgf@yb \advance\pgf@yc by-10pt
% construct main path
\pgfpathmoveto{\pgfpoint{\pgf@xa}{\pgf@ya}}
\pgfpathlineto{\pgfpoint{\pgf@xa}{\pgf@yb}}
\pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yb}}
\pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@yc}}
\pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@ya}}
\pgfpathclose
% add little corner
\pgfpathmoveto{\pgfpoint{\pgf@xc}{\pgf@yb}}
\pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
\pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@yc}}
\pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
}
}
\makeatother

\tikzstyle{doc}=[%
draw,
color=black,
shape=document,
shape=document,
inner sep=2ex,
]

